Galaxy Walker: Geometry-aware VLMs For Galaxy-scale Understanding

Modern vision-language models (VLMs) develop patch embedding and convolution backbone within vector space, especially Euclidean ones, at the very founding. When expanding VLMs to a galaxy scale for understanding astronomical phenomena, the integration of spherical space for planetary orbits and hyperbolic spaces for black holes raises two formidable challenges. a) The current pre-training model is confined to Euclidean space rather than a comprehensive geometric embedding. b) The predominant architecture lacks suitable backbones for anisotropic physical geometries. In this paper, we introduced Galaxy-Walker, a geometry-aware VLM, for the universe-level vision understanding tasks. We proposed the geometry prompt that generates geometry tokens by random walks across diverse spaces on a multi-scale physical graph, along with a geometry adapter that compresses and reshapes the space anisotropy in a mixture-of-experts manner. Extensive experiments demonstrate the effectiveness of our approach, with Galaxy-Walker achieving state-of-the-art performance in both galaxy property estimation ($R^2$ scores up to $0.91$) and morphology classification tasks (up to $+0.17$ F1 improvement in challenging features), significantly outperforming both domain-specific models and general-purpose VLMs.

==> figures/prompt_template_morphology1.tex <==
\begin{figure*}[t]
\begin{AIbox}{\DV: Galaxy Morphology Classification}
{\bf Prompt:}\\
{\scriptsize

Please tell me the given galaxy belongs to which morphology class? Here are $10$ questions that need to be answered. 
\begin{enumerate}
    \item The morphological class of a galaxy can be analyzed using multiple tokens: the morphological classification of galaxies, such as spiral, elliptical, or irregular, can be directly observed by analyzing their images. Spectral analysis reveals the motion and composition of stars and gas within the galaxy, aiding in understanding its structure. Spatial coordinates provide precise information about the position of the galaxy in the universe, and different geometric backgrounds (Euclidean, hyperbolic, and spherical) help refine and verify the morphological classification from various curvature perspectives. Specifically:
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} utilizes celestial images to assess the galaxy's overall shape and structural features, helping to classify it as smooth, featured, or an artifact.
        \item The \textbf{[Spectral token]} examines spectral lines to provide information on the galaxy’s composition and any distortions that might indicate its morphological class.
        \item The \textbf{[Euclidean token]} offers the galaxy's precise coordinates in flat space, allowing for spatial analysis and comparison with known morphological classes. 
        \item The \textbf{[Hyperbolic token]} provides insights into negative curvature space, aiding in the understanding of complex structures that might influence the galaxy's morphology.
        \item The \textbf{[Sphere token]} uses spherical geometry to interpret the galaxy's appearance in positively curved space, helping to refine its classification.
    \end{enumerate}
    \textbf{Please tell me which morphological class this galaxy belongs to}.
        \begin{enumerate}
            \item[(a)] Smooth.
            \item[(b)] Featured or Disk.
            \item[(c)] Artifact.
        \end{enumerate}
    \item Determining if a galaxy is disk-edge-on can be analyzed using multiple tokens: edge-on disk galaxies are characterized by their flat, edge-like appearance when observed. This can be directly identified from images. Spectral analysis can reveal the rotational velocity profile of the disk, confirming its edge-on orientation. Spatial coordinates, along with geometric backgrounds, help verify the galaxy’s orientation in the universe. Specifically:
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} offers visual information on the galaxy's edge-on appearance, which is indicative of a disk-edge-on orientation. 
        \item The \textbf{[Spectral token]} provides insights into the distribution of spectral lines, which might show rotation curves consistent with a disk-edge-on galaxy. 
        \item The \textbf{[Euclidean token]} gives the galaxy's precise coordinates in flat space, assisting in spatial orientation analysis. 
        \item The \textbf{[Hyperbolic token]} models the galaxy's structure in a negatively curved space, helping to understand any distortions that confirm its disk-edge-on nature. 
        \item The \textbf{[Sphere token]} uses spherical geometry to analyze the galaxy’s orientation in positively curved space. 
    \end{enumerate}
    \textbf{Please tell me if this is a disk-edge-on galaxy}.
        \begin{enumerate}
            \item[(a)] Yes, it is a disk-edge-on galaxy.
            \item[(b)] No, it is not a disk-edge-on galaxy.
        \end{enumerate}

    \item Determining if a galaxy has spiral arms can be analyzed using multiple tokens: spiral-arm galaxies typically exhibit distinct spiral patterns in images. Spectral analysis can reveal regions of new star formation and gas flow within the spiral arms. Spatial coordinates and geometric perspectives aid in understanding the spatial structure and distribution of these spiral arms. Specifically:
        \begin{enumerate}[label=$\circ$]
            \item The \textbf{[Image token]} provides visual information to identify the presence and patterns of spiral arms. 
            \item The \textbf{[Spectral token]} offers the analysis of the spectral lines, which may vary along the arms due to star formation activity. 
            \item The \textbf{[Euclidean token]} provides the galaxy’s coordinates in flat space, aiding in spatial relationship analysis of spiral structures. 
            \item The \textbf{[Hyperbolic token]} models the galaxy in a negatively curved space, providing geometric context for the spiral arms' formation. 
            \item The \textbf{[Sphere token]} uses spherical geometry to interpret the distribution and winding of spiral arms in positively curved space. 
        \end{enumerate}
    \textbf{Please tell me if this is a spiral-arms galaxy}.
        \begin{enumerate}
            \item[(a)] Yes, it is a spiral-arms galaxy.
            \item[(b)] No, it is not a spiral-arms galaxy.
        \end{enumerate}
    \item Determining the type of bar in a galaxy can be analyzed using multiple tokens: bar structures in galaxies can be directly observed through images, revealing their length and strength. Spectral analysis provides information on the effect of the bar on the dynamics of stars and gas within the galaxy. Spatial coordinates and geometric backgrounds further confirm the presence and type of the bar by providing additional context. Specifically: 
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} offers visual information to observe and classify the bar's strength in the galaxy. 
        \item The \textbf{[Spectral token]} provides analysis of spectral lines which could show the dynamics affected by the bar. 
        \item The \textbf{[Euclidean token]} gives the galaxy’s position in flat space, assisting in the spatial analysis of the bar. 
        \item The \textbf{[Hyperbolic token]} helps model the galaxy's structure in negatively curved space, which aids in understanding the bar type. 
        \item The \textbf{[Sphere token]} uses spherical geometry to analyze the distribution of stellar masses in the bar, refining its classification.
    \end{enumerate}
    \textbf{Please tell me which type of bar this galaxy has.}
        \begin{enumerate}
            \item[(a)] Strong Bar. 
            \item[(b)] Weak Bar.
            \item[(c)] No Bar.
        \end{enumerate}    
\end{enumerate}
}

{\bf \DV:}\\
{\scriptsize
[Predicted results for each question.]
}
\end{AIbox}
\vspace{-1em}
\caption{Prompt template of the galaxy morphology classification.}
\label{fig:prompt_template_morphology1}
\end{figure*}

==> figures/prompt_template_morphology2.tex <==
\begin{figure*}[t]
\begin{AIbox}{\DV: Galaxy Morphology Classification}
{\bf Prompt:}\\
{\scriptsize

Please tell me the given galaxy belongs to which morphology class? Here are $10$ questions that need to be answered. 
\begin{enumerate}[start=5]
    \item Determining the bulge size of a galaxy can be analyzed using multiple tokens: the size of a galaxy's bulge can be observed in images by its prominence. Spectral analysis reveals distinct characteristics of stars in the bulge such as age and composition, aiding in understanding its size. Spatial coordinates and different geometric backgrounds allow precise measurement and context for the bulge. Specifically: 
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} provides visual information to assess the bulge's prominence in the galaxy. 
        \item The \textbf{[Spectral token]} analyzes the stellar population's spectral lines to derive insights about the bulge’s age and composition. 
        \item The \textbf{[Euclidean token]} offers the galaxy’s coordinates in flat space, assisting in spatial analysis of the bulge's physical size. 
        \item The \textbf{[Hyperbolic token]} models the galaxy in negatively curved space, which helps in understanding the bulge size in a broader context. 
        \item The \textbf{[Sphere token]} uses spherical geometry to analyze the distribution and density of stars within the bulge.
    \end{enumerate}
    \textbf{Please tell me the bulge size of this galaxy}.
        \begin{enumerate}
            \item[(a)] Dominant Bulge.
            \item[(b)] Large Bulge.
            \item[(c)] Moderate Bulge.
            \item[(d)] Small Bulge.
            \item[(f)] No Bulge.
        \end{enumerate}

    \item Determining the shape of a galaxy can be analyzed using multiple tokens: the shape of a galaxy can be directly observed by analyzing its images. Spectral analysis reveals motion and composition differences that help understand the internal structure. Spatial coordinates and geometric backgrounds provide additional dimensions to confirm shape classification. Specifically:
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} provides visual information to classify the galaxy as round, in-between, or cigar-shaped. 
        \item The \textbf{[Spectral token]} analyzes observable spectral features that may be associated with different galaxy shapes. 
        \item The \textbf{[Euclidean token]} gives the galaxy's precise coordinates in flat space, aiding in the geometric analysis of its shape. 
        \item The \textbf{[Hyperbolic token]} models the galaxy’s structure in negatively curved space, providing a complex geometric context for its shape classification. 
        \item The \textbf{[Sphere token]} uses spherical geometry to analyze the galaxy’s three-dimensional shape in positively curved space.
    \end{enumerate}
    \textbf{Please tell me the shape of this galaxy}.
        \begin{enumerate}
            \item[(a)] Round.
            \item[(b)] In-Between.
            \item[(c)] Cigar-Shaped.
        \end{enumerate}

    \item Determining the type of bulge in an edge-on galaxy can be analyzed using multiple tokens: the type of bulge in an edge-on galaxy can be identified by observing its images, which show whether it is boxy or rounded. Spectral analysis provides information about the bulge's stellar composition and structure. Spatial coordinates and geometry help in confirming the type of bulge through a more detailed spatial analysis. Specifically:
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} gives visual information to identify and classify the bulge as boxy, rounded, or absent in an edge-on galaxy. 
        \item The \textbf{[Spectral token]} analyzes the spectral lines to provide insights into the bulge’s structural composition. 
        \item The \textbf{[Euclidean token]} offers the galaxy’s coordinates in flat space, assisting in the spatial analysis of the bulge. 
        \item The \textbf{[Hyperbolic token]} models the galaxy in negatively curved space, helping to understand the bulge type in a broader geometrical context. 
        \item The \textbf{[Sphere token]} uses spherical geometry to analyze the three-dimensional distribution of stars within the bulge.
    \end{enumerate}
    \textbf{Please tell me the type of bulge in this edge-on galaxy}. 
        \begin{enumerate}
            \item[(a)] Boxy Bulge.
            \item[(b)] No Bulge.
            \item[(c)] Rounded Bulge.
        \end{enumerate}
        
    \item Analyzing how tightly wound the spiral arms of a galaxy can be done using multiple tokens: the tightness of spiral arms can be directly observed in images, showing the winding patterns clearly. Spectral analysis reveals variations in stars' compositions along the arms, indicative of different winding levels. Spatial coordinates and geometry provide additional context for analyzing the winding of the arms in greater detail. Specifically:
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} provides visual information to determine the tightness of the spiral arms. 
        \item The \textbf{[Spectral token]} analyzes variations in spectral lines along the arms, which may indicate differing winding levels. 
        \item The \textbf{[Euclidean token]} gives the galaxy's precise coordinates in flat space, aiding in the spatial analysis of spiral arm winding. 
        \item The \textbf{[Hyperbolic token]} models the galaxy’s structure in negatively curved space, helping to understand the geometric properties affecting spiral arm tightness. 
        \item The \textbf{[Sphere token]} uses spherical geometry to analyze the three-dimensional winding of the spiral arms.
    \end{enumerate}
    \textbf{Please tell me how tightly wound the spiral arms of this galaxy are}.
        \begin{enumerate}
            \item[(a)] Tight Winding.
            \item[(b)] Medium Winding.
            \item[(c)] Loose Winding.
        \end{enumerate}

\end{enumerate}
}

{\bf \DV:}\\
{\scriptsize
[Predicted results for each question.]
}
\end{AIbox}
\vspace{-1em}
\caption{Prompt template of the galaxy morphology classification.}
\label{fig:prompt_template_morphology2}
\end{figure*}

==> figures/prompt_template_morphology3.tex <==
\begin{figure*}[t]
\begin{AIbox}{\DV: Galaxy Morphology Classification}
{\bf Prompt:}\\
{\scriptsize

Please tell me the given galaxy belongs to which morphology class? Here are $10$ questions that need to be answered. 
\begin{enumerate}[start=9]
    
    \item Determining the number of spiral arms in a galaxy can be analyzed using multiple tokens: the number of spiral arms in a galaxy can be directly counted from images. Spectral analysis helps trace the stellar distribution in each arm. Spatial coordinates and geometric contexts provide additional details for a precise count and understanding of the distribution. Specifically:
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} provides visual information to count and identify the number of spiral arms. 
        \item The \textbf{[Spectral token]} analyzes spectral lines to trace the distribution of stars in spiral arms. 
        \item The \textbf{[Euclidean token]} gives the galaxy's precise coordinates in flat space, aiding in the spatial analysis of the spiral arms. 
        \item The \textbf{[Hyperbolic token]} models the galaxy’s structure in negatively curved space, providing a geometric context for the number of spiral arms. 
        \item The \textbf{[Sphere token]} uses spherical geometry to analyze the three-dimensional distribution of spiral arms.
    \end{enumerate}
    \textbf{Please tell me the number of spiral arms in this galaxy}.
        \begin{enumerate}
            \item[(a)] 1 Spiral Arm.
            \item[(b)] 2 Spiral Arms.
            \item[(c)] 3 Spiral Arms.
            \item[(d)] 4 Spiral Arms.
            \item[(e)] More than 4 Spiral Arms.
            \item[(f)] Can't Tell.
        \end{enumerate}
    \item Determining the merging state of a galaxy can be analyzed using multiple tokens: the merging state of a galaxy can be observed through signs of disturbance or merging in images. Spectral analysis reveals interactions between stars and gas at different merging stages. Spatial coordinates and geometric analysis provide comprehensive insights into the merging process. Specifically:
    \begin{enumerate}[label=$\circ$]
        \item The \textbf{[Image token]} provides visual information to observe signs of merging or disturbances. 
        \item The \textbf{[Spectral token]} analyzes variations in spectral lines to detect interactions indicative of different merging states. 
        \item The \textbf{[Euclidean token]} offers the galaxy’s coordinates in flat space, aiding in assessing merging stages from spatial data. 
        \item The \textbf{[Hyperbolic token]} models the galaxy in negatively curved space, helping to understand the geometric properties affecting the merging state. 
        \item The \textbf{[Sphere token]} uses spherical geometry to analyze the three-dimensional interactions of merging galaxies.
    \end{enumerate}
    \textbf{Please tell me the merging state of this galaxy}.
        \begin{enumerate}
            \item[(a)] No Merging.
            \item[(b)] Minor Disturbance.
            \item[(c)] Major Disturbance.
            \item[(d)] Merger.
        \end{enumerate}
    
\end{enumerate}
}

{\bf \DV:}\\
{\scriptsize
[Predicted results for each question.]
}
\end{AIbox}
\caption{Prompt template of the galaxy morphology classification.}
\label{fig:prompt_template_morphology3}
\end{figure*}

==> figures/prompt_template_property.tex <==
\begin{figure*}[t]
\begin{AIbox}{\DV: Galaxy Property Estimation}
{\bf Prompt:}\\
{\scriptsize
Stellar mass refers to the total mass of all the stars in a galaxy. It is a critical parameter for understanding galaxy formation and evolution and can be analyzed through multiple perspectives. Specifically, the \textbf{[Image token]} utilizes celestial image data to assess morphology and luminosity, which helps in the initial estimation of stellar mass. The \textbf{[Spectral token]} analyzes stellar spectral characteristics, such as absorption line width and radiation intensity, to directly infer mass parameters. The \textbf{[Euclidean token]} provides the object's position in flat space, aiding in the mass calculation by considering distance measurements. The \textbf{[Hyperbolic token]} describes the geometrical properties in negatively curved space, modeling more complex cosmic structures and helping to understand the distribution of massive stars in a negatively curved universe. The \textbf{[Sphere token]} uses spherical geometry in positively curved space to evaluate an object's position in the spherical coordinate system, leading to a more accurate mass estimation. \textbf{By integrating information from these tokens, please tell me the Stellar Mass}. 
}\\

{\bf \DV:}\\
{\scriptsize
[The prediction of the stellar mass.]
} \\

{\bf Prompt:}\\
{\scriptsize
Mass-weighted stellar metallicity measures the abundance of elements heavier than hydrogen and helium in a galaxy's stars, weighted by their mass. This aids in understanding the galaxy's chemical evolution and can be analyzed through multiple perspectives. Specifically, the \textbf{[Image token]} helps observe the color and brightness variations of celestial objects, providing initial metallicity estimates. The \textbf{[Spectral token]} offers a detailed analysis of spectral lines, such as the strength and shift of metal lines, to directly infer the mass-weighted metallicity. The \textbf{[Euclidean token]} provides precise coordinates in flat space, aiding in the calculation of metallicity distribution within stars by using distance information. The \textbf{[Hyperbolic token]} describes the geometrical properties in negatively curved space, modeling complex star cluster structures and giving geometrical background support for metallicity distribution. The \textbf{[Sphere token]} employs spherical geometry in positively curved space to understand the distribution of celestial objects within the spherical coordinate system, leading to comprehensive metallicity estimation. \textbf{By integrating information from these tokens, please tell me the Mass-Weighted Stellar Metallicity}. 
}\\

{\bf \DV:}\\
{\scriptsize
[The prediction of the mass-weighted stellar metallicity.]
}\\

{\bf Prompt:}\\
{\scriptsize
Mass-weighted galaxy age refers to the average age of stars within a galaxy, weighted by their mass, providing insights into the galaxy's formation history. This can be analyzed through multiple perspectives. Specifically, the \textbf{[Image token]} assesses morphology and color via celestial images to estimate the age distribution of stellar populations in the galaxy. The \textbf{[Spectral token]} primarily uses spectral analysis, such as examining the spectral energy distribution and absorption line changes, to determine the overall age of the galaxy. The \textbf{[Euclidean token]} provides the galaxy's coordinates in flat space, assisting in refining age estimation based on distance and position. The \textbf{[Hyperbolic token]} describes complex geometrical backgrounds in negatively curved space, aiding in the detailed understanding of mass-weighted age composition. The \textbf{[Sphere token]} utilizes positively curved space in spherical geometry to assist in distribution analysis and age estimation of different regions within the galaxy. \textbf{By integrating information from these tokens, please tell me its Mass-Weighted Galaxy Age (Gyr)}.
}\\

{\bf \DV:}\\
{\scriptsize
[The prediction of the mass-weighted galaxy age (Gyr).]
}\\

{\bf Prompt:}\\
{\scriptsize
The specific star-formation rate (sSFR) is the rate of star formation per unit stellar mass in a galaxy, indicating how actively the galaxy is forming stars relative to its existing stellar mass. It can be analyzed through multiple perspectives. Specifically, the \textbf{[Image token]} helps analyze star-forming regions, morphology, and density variations via celestial images for initial estimation of the star-formation rate. The \textbf{[Spectral token]} provides detailed spectral analysis, especially the intensity and distribution of emission lines, to measure the current star-formation rate. The \textbf{[Euclidean token]} offers precise positioning in flat space, aiding in inferring the star-formation rate based on distance and velocity information. The \textbf{[Hyperbolic token]} describes geometrical properties in negatively curved space, modeling complex cosmic environments and star cluster structures for supporting star-formation rate estimation. The \textbf{[Sphere token]} utilizes positively curved space in spherical geometry to understand the distribution of star formation within the spherical coordinate system, assisting in specific rate determination. \textbf{By integrating information from these tokens, please tell me its Specific Star-Formation Rate}.
}\\

{\bf \DV:}\\
{\scriptsize
[The prediction of Specific Star-Formation Rate.]
}
\end{AIbox}
\caption{Prompt template of the galaxy property estimation.}
\label{fig:prompt_template_property}
\end{figure*}

==> figures/prompt_template_redshift.tex <==
\begin{figure*}[t]
\begin{AIbox}{\DV: Redshift Estimation}
{\bf Prompt:}\\
{\scriptsize
Redshift is a measure of how much the wavelength of light from a galaxy has been stretched due to the expansion of the universe. It provides crucial information on the galaxy's velocity and distance and can be analyzed through multiple perspectives. Specifically, the \textbf{[Image token]} utilizes celestial image data to obtain observational information such as morphology and luminosity, providing an initial estimate of distance. The \textbf{[Spectral token]} directly calculates the redshift value through the displacement of spectral lines. The \textbf{[Euclidean token]} offers spatial coordinates in Euclidean space, aiding in the calculation of the celestial object's position and distance. The \textbf{[Hyperbolic token]} describes more complex cosmic structures, providing additional geometric context. The \textbf{[Sphere token]} utilizes spherical geometry information to understand the object's position in a spherical coordinate system, aiding in distance determination. \textbf{By integrating the information from these tokens, we derive the redshift value of the celestial object}. 
}\\

{\bf \DV:}\\
{\scriptsize
[The prediction of redshift.]
}
\end{AIbox}
\caption{Prompt template of the redshift estimation.}
\label{fig:prompt_template_redshift}
\end{figure*}

==> sec/3_prelimianries.tex <==
\section{Preliminaries}
\subsection{Riemannina Geometry}
A smooth manifold $M^d$ is referred to as a Riemannian manifold when it possesses a Riemannian metric $g$, where $d$ denotes its dimension. For each point $x \in M$, there exists a tangent space $T_xM^d \subseteq \mathbb{R}^d$ that surrounds $x$, where the metric $g$ is applied to determine the manifold's shape. The relationship between the tangent space and the manifold is established through the use of exponential and logarithmic maps. In particular, the logarithmic map at point $x$, represented as $\log_x(\cdot): M \to T_xM$, transforms points from the manifold into the tangent space, while the exponential map functions inversely.

Curvature serves as a crucial measure of the degree of curvature in Riemannian geometry. When curvature is zero, geodesics remain parallel; positive curvature causes geodesics to converge, while negative curvature leads to their divergence. Hyperbolic spaces exhibit negative curvature, whereas hyperspherical spaces exhibit positive curvature. The relevant operator definitions are provided in Table 1.


% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c|c|c}
%         \toprule
%         \textbf{Space Model} & $\exp_{x_p}(x)$ & $\mathcal{D}(x, y)$ \\
%         \midrule
%         Euclidean(E) & $x_p + x$ & $\|x - y\|_2$ \\
%         Hyperboloid(H) & $\cosh\left( \sqrt{-K_H} \|x\|\right) x_p + \sinh\left( \sqrt{-K_H} \|x\| \right) \frac{x}{\sqrt{-K_H} \|x\|}$ & $\frac{1}{\sqrt{-K_H}} \operatorname{arccosh} (K_H \langle x, y \rangle /c)$ \\
%         Hypersphere(S) & $\cos\left( \sqrt{K_S} \|x\|\right) x_p + \sin\left( \sqrt{K_S} \|x\| \right) \frac{x}{\sqrt{K_S} \|x\|}$ & $\frac{1}{\sqrt{K_S}} \operatorname{arccos} (K_S \langle x, y \rangle)$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Space Model Comparison}
% \end{table}
